Robust Two-View Geometry Estimation with Implicit Differentiation

We present a novel two-view geometry estimation framework which is based on a differentiable robust loss function fitting. We propose to treat the robust fundamental matrix estimation as an implicit layer, which allows us to avoid backpropagation through time and significantly improves the numerical stability. To take full advantage of the information from the feature matching stage we incorporate learnable weights that depend on the matching confidences. In this way our solution brings together feature extraction, matching and two-view geometry estimation in a unified end-to-end trainable pipeline. We evaluate our approach on the camera pose estimation task in both outdoor and indoor scenarios. The experiments on several datasets show that the proposed method outperforms both classic and learning-based state-of-the-art methods by a large margin. The project webpage is available at: https://github.com/VladPyatov/ihls

==> sections/1_intro.tex <==
%\input{preamble}
\section{INTRODUCTION}
\label{sec:intro}

Nowadays, 3D computer vision has received widespread attention and has found application in a wide range of tasks, including scene reconstruction \cite{Schonberger_2016_CVPR,Wang_2021_CVPR,Xiao_2023_CVPR}, autonomous driving \cite{Prakash_2021_CVPR, Hu_2023_CVPR, Deng_2023_ICCV}, neural rendering~\cite{mildenhall2020nerf} %, Sucar_2021_ICCV, Bian_2023_CVPR}  
and map-free re-localization \cite{arnold2022mapfree}. To deal with such tasks a  first necessary step is to recover the position and orientation of each camera in the scene or equivalently to solve the Camera Pose Estimation (CPE) problem \cite{Schonberger_2016_CVPR, Jau_2020_IROS, Parameshwara_2022_CVPR, Roessle_2023_ICCV}.

Given a set of input images, the solution of CPE typically consists of three essential steps. First, putative keypoint correspondences are established through the feature extraction \cite{Lowe_2004, Yi_2016, DeTone2017SuperPointSI, Tyszkiewicz_2020_NeurIPS} and matching \cite{Sarlin_2020_CVPR, Sun_2021_CVPR, chen2022aspanformer} stages. The second step involves the recovery of the two-view geometry \cite{hartley_zisserman_2004, Szeliski2022, Barroso-Laguna_2023_CVPR} by estimating the relative camera poses between image pairs. This estimate provides a good initial solution that is later refined by bundle adjustment \cite{Triggs1999BundleA, Agarwal_2010_ECCV, tang2018banet, Huang_2021_CVPR, Weber_2023_CVPR} in the final stage. 
%Bundle adjustment which boils down to a joint nonlinear optimization of the 3D coordinates of the extracted features and pose parameters of all cameras in the scene. 
The feature matching and bundle adjustment problems have received a lot of attention over the past few years, especially with the advent of learning-based approaches. At the same time two-view geometry estimation, though it plays an important role in Bundle Adjustment and significantly influences the result of the aforementioned tasks, has not been widely studied.

The two-view geometry of an image pair is usually represented either with an essential \cite{LonguetHiggins1981ACA} or (in the uncalibrated camera setup) a fundamental matrix \cite{Faugeras1992WhatCB} that define an algebraic representation of the geometric epipolar constraint \cite{hartley_zisserman_2004}. These matrices can be estimated from a set of putative keypoint correspondences using the \textit{least squares} approach. However, due to occlusions, repetitive patterns, illumination changes and poor textures present in a scene, the feature matching stage may produce outliers, mismatched pairs that affect the solution and, above all, lead to an incorrect geometry representation. Given that the least squares method works under the assumption that the noise in the matches obeys a Gaussian distribution, it is unable to efficiently handle severe outliers and can lead to poor estimation results. 
% This issue has gained the attention of the research community and initiated the seek of alternatives and the investigate the direction of outlier-robust model estimation}.

One possible way to deal with outliers is to utilize RANSAC-based estimators \cite{RANSAC, Torr_2000, Chum2003LocallyOR, Chum2005TwoviewGE, Barath_2018_CVPR, Barath_2019_CVPR, Barath_2020_CVPR}. The main strategy followed by these methods is based on the hypothesize-and-verify approach. Specifically, after the feature matching stage, minimal subsets of the putative matches are randomly sampled and the corresponding two-view geometries are estimated with either the 8-\cite{LonguetHiggins1981ACA} 7- \cite{Hartley_1994_TPAMI} or 5-point \cite{Nister_2004_TPAMI} algorithms in order to form a pool of model hypotheses. Then the generated hypotheses are scored by counting the number of inliers, \ie matches with residual error below a selected threshold. Finally, the best model hypothesis is further refined by using all the inlier correspondences. Despite their effectiveness, the non-deterministic nature of RANSAC-based estimators precludes efficient end-to-end training when neural networks are involved in the overall pipeline. As a consequence, taking full advantage of the information available from the feature extraction and matching stages becomes challenging.

Another line of work that aims to circumvent the problems appearing due to outliers, is devoted to the introduction of robust loss functions \cite{Torr1997TheDA, ruckstuhl2014, Barron_2019_CVPR}, a specific type of M-estimators \cite{Huber1964RobustEO, Huber2005RobustS}. According to this approach, the solution to the two-view geometry problem is obtained by optimizing an objective function that is less sensitive to the presence of outliers. In general, the task is formulated as a non-convex and possibly non-smooth optimization problem that is typically solved employing iterative numerical algorithms \cite{Peng_2023_CVPR}. In general, given the non-convex nature of the objective, the solution is not guaranteed to attain the global minimum, but in practice if the fraction of outliers is relatively small, then the recovered two-view geometry is more precise compared to the one estimated with RANSAC-based methods. On the other hand, when the outlier pairs start dominating the correspondences, the solution becomes sub-optimal and hurts the performance of the downstream tasks. 

The learning-based approach in~\cite{Ranftl_2018_ECCV} tries to alleviate this problem by aiming to implicitly learn a robust loss function. However, this method faces the important limitation of having to back-propagate through unrolled layers that involve the singular value decomposition (SVD). This leads both to an increased memory footprint during training as well as numerical instabilities mostly from the back-propagation through SVD. Because of these reasons the authors of~\cite{Ranftl_2018_ECCV} limit the number of the employed unrolled layers to just a few, which in turn hinders the final performance of their approach. 

In this work we revisit the direction of robust loss function fitting and propose a novel approach for outlier-robust two-view geometry estimation problem. First, we adopt a specific parametric form for the robust loss that exhibits several important benefits both in terms of robustness to outliers and efficiency in training. 
%make a step away from conventional IRLS-based robust function fitting definition and reformulate the optimizaiton problem in a well-defined way that ensures convergence guaranties. 
To successfully minimize this non-convex loss we introduce the Iterative Homogeneous Least Squares (IHLS) solver that takes as input putative keypoint correspondences and outputs an estimate of the underlying two-view geometry. To avoid back-propagation through IHLS with unrolling, we take advantage of the convergence guaranties of our solver and utilize the implicit function theorem that allows us to perform back-propagation without the need to save any intermediate results from the forward pass or back-propagate through the SVD layer, which is an essential part of our optimization algorithm. Further, to downplay the role of the outliers, we develop a learnable framework on top of the IHLS solver and utilize a weight prediction network that re-estimates matching confidences in a recurrent fashion based on the matches, residuals of the current solution and auxiliary information from the feature matching stage. We then chain our framework with the LoFTR \cite{Sun_2021_CVPR} dense feature matching transformer to obtain a fully differentiable robust camera pose estimation pipeline. To summarize, our main contributions are as follows:
\begin{itemize}%[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item We employ a robust parametric loss function to deal with the fundamental matrix estimation problem and propose the Iterative Homogeneous Least Squares solver which can efficiently recover a solution of the underlying minimization problem. 
    \item The convergence guaranties of IHLS further allows us to introduce an efficient end-to-end training strategy using implicit backpropagation, which significantly reduces the memory requirements and improves the stability of training compared to alternative approaches that employ unrolled networks.
    %\item We propose the Iterative Homogeneous Least Squares solver to facilitate learning-based robust loss function fitting
    \item We propose an end-to-end trainable camera pose estimation pipeline that brings together feature extraction, matching and robust two-view geometry estimation.
    \item Extensive experiments on both outdoor and indoor data demonstrate that our method not only outperforms existing approaches, but also improves the performance of the feature matching network itself.
\end{itemize}

==> sections/2_related_work.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/framework_modified.pdf}
    \caption{Overview of the proposed end-to-end trainable framework. The pair of source and target images $\bm I_S, \bm I_T$ is passed through the LoFTR feature extraction module to predict the set of correspondences $\bm p$ and a context vectors $\bm \tau$. Both are then used to initialize and guide the fundamental/essential matrix estimation via the proposed recurrent strategy consisting of refinement network and IHLS solver. For detailed description of please refer to Sec.~\ref{sec:method}.}
    \label{fig:framework}
    \vspace{-0.5cm}
\end{figure*}

\section{RELATED WORK}
\label{sec:related_work}

\subsection{Feature extraction and matching}
Hand-crafted local features, such as SIFT \cite{Lowe_2004} and ORB \cite{Rublee_2011}, combined with a mutual nearest neighbour search or Lowe's ratio test \cite{Lowe_2004} have been considered as the dominant correspondence estimation approach for a long time. Nevertheless, with the advent of deep learning the components of the classic pipeline have been largely revisited. In particular, learning-based local features \cite{Yi_2016, DeTone_2017, DeTone2017SuperPointSI, Barroso-Laguna_2019_ICCV} show impressive results in challenging conditions of viewpoint change and poor texture. SuperGlue \cite{Sarlin_2020_CVPR} proposes a learning-based approach for local feature matching on top of the sparse SuperPoint \cite{DeTone2017SuperPointSI} features, while the recently introduced LightGlue \cite{lindenberger2023lightglue} further reduces its computational complexity. LoFTR \cite{Sun_2021_CVPR} and its successors \cite{chen2022aspanformer, yu2023adaptive, Yu_2023_CVPR, Huang_2023_CVPR} take advantage of dense feature extraction and propose a detector-free design.

\subsection{RANSAC-based estimators}
RANSAC-based approaches either try to improve hypothesis scoring of the original RANSAC \cite{RANSAC} or propose end-to-end trainable counterparts. MLESAC \cite{Torr_2000} chooses the solution that maximizes the likelihood rather than just the number of inlier pairs and thus is less sensitive to the inlier threshold. LO-RANSAC \cite{Chum2003LocallyOR} applies local optimization to the so-far-the-best model hypothesis. DEGENSAC \cite{Chum2005TwoviewGE} detects degenerate configurations and rejects models that are incompatible with the scene geometry. MAGSAC \cite{Barath_2019_CVPR} proposes to marginalize the quality function over a range of noise levels to eliminate the threshold from the model quality calculation.  State-of-the-art approach MAGSAC++ \cite{Barath_2020_CVPR} proposes a novel marginalization procedure and introduces a new model quality function that does not require the inlier-outlier decision. On the other hand, inspired by the success of reinforcement learning, DSAC \cite{Brachmann_2017_CVPR, brachmann2018lessmore, brachmann2021dsacstar} methods introduce a first learning-based alternative and incorporate REINFORCE \cite{Williams_1992} algorithm to make the hypothesis selection procedure differentiable. Neural-guided RANSAC \cite{Brachmann_2019_ICCV} makes a step forward and proposes learned guidance of hypothesis sampling. Barath \etal \cite{Barath_2022_CVPR} replaces conventional hypothesis scoring with MQ-Net that predicts model quality based on the residual histogram and additionally plugs in MF-Net for early rejection of degenerate models. $\nabla$-RANSAC \cite{Wei_2023_ICCV} revises the learning-based problem formulation and incorporates the Gumbel Softmax \cite{jang2017categorical} relaxation to estimate the gradients in the sampling distribution.

\subsection{Robust loss functions} 
Robust loss functions serve as an alternative strategy for outlier-robust model fitting and is the main focus of this work. Since their introduction in the context of M-estimators \cite{Huber1964RobustEO}, their applicability to the two-view geometry estimation \cite{MacTavish_2015_AtAC} has been proven. The aforementioned MAGSAC++ \cite{Barath_2020_CVPR} reformulates the model fitting problem as an M-estimation and solves it with an iteratively reweighted least squares (IRLS) procedure. To downplay the role of outliers Ranfl and Koltun \cite{Ranftl_2018_ECCV} proposed to cast the robust function learnable and simulated the IRLS procedure in their Deep Fundamental Matrix Estimation (DFE) approach. In attempts to overcome the limitations of IRLS, Ikami \etal \cite{Ikami_2018_CVPR} developed a novel objective function and proposed the iteratively reweighted eigenvalues minimization (IREM) for its optimization.



==> sections/_3.1_algo_is_not_used.tex <==
\subsection{Iterative Homogeneous Least Squares}
\label{sec:IHLS}

In this section we describe in detail our approach for solving the optimization problem of interest. To proceed, we utilize
the following inequality~\cite{Sun2016}:
\bal
\abs{f}^p \le \frac{p}{2}\frac{f^2}{\beta^{2-p}} + \frac{2-p}{2}\beta^p,
\label{eq:lp_ineq}
\eal
which holds true $\forall f\in \R$, $\beta > 0$ and $0<p\le 2$.

Let us now consider the positive scalar $ \sqrt{f_n^2+ \epsilon} $ with $ \epsilon >0 $ being a small positive constant and plug it in ~\eqref{eq:lp_ineq}. Then, we obtain
\bal
\pr{f_n^2+\epsilon}^{\frac{p}{2}} \le \frac{p}{2}\frac{f_n^2}{\beta_n^{2-p}}+\frac{p\epsilon}{2}\beta_n^{p-2}+ \frac{2-p}{2}\beta_n^p.
\label{eq:lp_gamma_ineq}
\eal
The above inequality is closed under summation and, thus, it further holds that:
\bal
\rho\pr{\bm f;\epsilon, p}=&\suml_{n=1}^N \pr{f_n^2+\epsilon}^{\frac{p}{2}}
\le \frac{p}{2}\bm f^\transp\pdiag{\bm\beta}{p-2}\bm f\nonumber\\
+&\suml_{n=1}^N\pr{\frac{p\epsilon}{2}\beta_n^{p-2}+\frac{2-p}{2}\beta_n^p}=\psi\pr{\bm\beta}.
\eal
Moreover, by noting that all the terms of $\psi\pr{\bm\beta}$ are strictly positive, we end up with the following identity 
\bal
\rho\pr{\bm f;\epsilon, p} =\min_{\bm\beta\in\R^N_+} \psi\pr{\bm\beta},
\label{eq:var_beta}
\eal
which can be easily verified by differentiating w.r.t $\bm\beta$.
We have, thus, managed to obtain a variational formulation of the robust function $\rho\pr{\bm f;\epsilon, p}$ as the minimum of a quadratic function in $\bm f$ over the auxiliary variable $\bm \beta$.

Combining ~\eqref{eq:argmin_f} and \eqref{eq:var_beta} we get:
\bal
\min_{\norm{\bm f}{}=1}&\rho\pr{\m A\bm x;\epsilon,p}=\min_{\norm{\bm f}{}=1,\,\bm\beta\in\R^N_+} \phi\pr{\bm f, \bm\beta} \equiv\nonumber\\&\frac{p}{2}\bm f^\transp\bm \Gamma\pr{\bm\beta}\bm f+\suml_{n=1}^N\pr{\frac{p\epsilon}{2}\beta_k^{p-2}+\frac{2-p}{2}\beta_k^p},
\label{eq:min_min}
\eal
where 
\bal
\bm\Gamma\pr{\bm\beta}=\m A^\transp\pdiag{\bm\beta}{p-2}\m A = \m A^\transp\m B\m A.
\label{eq:Gamma_mat}
\eal
By exploiting the variational formulation of~\eqref{eq:var_beta} we have achieved to express our original problem in~\eqref{eq:argmin_f} as a joint minimization in the variables $\pr{\bm f, \bm \beta}$, for which it is possible to consider the following alternating minimization strategy:
\begin{subequations}
\label{eq:cyclic_min}
\bal
\begin{split}\label{eq:beta_min}
\bm\beta^{k+1}&=\argmin_{\bm\beta\in\R^N_+}\phi\pr{\bm f^k,\bm\beta},
\end{split}\\
\begin{split}\label{eq:x_min}
\bm f^{k+1}&=\argmin_{\norm{\bm x}{}=1}\phi\pr{\bm f,\bm\beta^{k+1}}.
\end{split}
\eal
\end{subequations}

The minimizer of~\eqref{eq:beta_min} can be found by equating the gradient of the respective objective to zero, $\grad{\phi\pr{\bm f^k;\bm\beta}}{\bm\beta}=\bm 0$, which takes the form:
\bal
\kappa\pr{\pdiag{\m A\bm f^k}{2}+\epsilon\bm I - \pdiag{\bm\beta}{2}}\bm\beta^{p-3} = \bm 0,
\label{eq:beta_system}
\eal
where $\kappa=p(p-2)/2$.
For the case of interest $0 < p \le 1$ and given that $\beta_n$ is constrained to be strictly positive, the only admissible solution of Eq.~\eqref{eq:beta_system} is 
\bal
\beta_n^{k+1}=\sqrt{\pr{\bm e_n^\transp\m A\bm f^k}^2+\epsilon},\,\,\forall n=1,\ldots, N,
\label{eq:beta_k}
\eal
with $\bm e_n$ denoting the unit vector of the standard $\R^N$ basis, \ie all its elements are zero except to the $n$-th one which is equal to one.

Next, we notice that the minimizer of~\eqref{eq:x_min} corresponds to the solution of a unit-norm constrained homogeneous least-squares problem~\cite{Szeliski2022}. This solution is expressed as:
\bal
\bm f^{k+1} = \bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta^{k+1}}},
\label{eq:f_argmin_beta}
\eal
where $\bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta^{k+1}}}$ denotes the eigenvector corresponding to the smallest eigenvalue of the symmetric and positive definite matrix $\bm\Gamma\pr{\bm\beta^{k+1}}$. 

Finally, by combining~\eqref{eq:Gamma_mat}, \eqref{eq:beta_k}, and \eqref{eq:f_argmin_beta}, the overall minimization algorithm can be written in the compact form:
\bal
\label{eq:forward_iterations}
%\bm x^{k+1}&=\bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta^{k+1}}}\nonumber\\
\bm f^{k+1}=\bm u_{\text{min}}\pr{\m A^\transp \pdiag{\pr{\m A\bm f^k}^2 + \epsilon\bm I}{\frac{p-2}{2}}\m A}.
\eal
The derived update strategy corresponds to an iterative homogeneous least-squares solver (IHLS), where in each iteration $k\!+\!1$ the involved diagonal matrix $\m B^k=\pdiag{\pr{\m A\bm f^k}^2 + \epsilon\bm I}{\frac{p-2}{2}}$ is updated according to the solution of the previous iteration, $\bm f^k$.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/ihls_layer.pdf}
    \caption{The proposed IHLS layer architecture.}
    \label{fig:ihls}
\end{figure}

\subsection{Network Training} %with Implicit Backpropagation}
\label{sec:backward_pass}
% Being our final goal, supervised end-to-end learning of geometry parameters requires backpropagation through the iterative procedure described by~\cref{eq:forward_iterations}. Its recurrent nature suggests us to represent it as a recurrent layer, whose parameters $\m A$ are predicted by the preceding features extraction and matching module. The resulting layer consists of three sequential operations, namely:
% \begin{itemize}
%     \item \textbf{Residual computation}, that gets as input the current estimate $\bm x^k$ and computes the residual vector $\bm r^k = \m A \bm x^k$.
%     \item \textbf{Normal equations matrix computation}, which constructs the matrix $\m A^k = \m A^\transp \pdiag{\pr{\bm r^k}^2 + \epsilon\bm I}{\frac{p-2}{2}}\m A$.
%     \item \textbf{Constrained least squares solution}, which computes the updated estimate $\bm x^{k+1} = \bm u_{\text{min}}\pr{\m A^k}$ by solving the constrained least squares with normal equations matrix $\m A^k$ by finding the eigenvector corresponding to the smallest eigenvalue of $\m A^k$.
% \end{itemize}
% We present the overall architecture of the 
Our final goal is to employ the IHLS solver as a layer in a wider network, which will be trained end-to-end in a supervised way. To do so, we need to be able to back-propagate efficiently through the IHLS layer. The main challenge here is that the proposed IHLS solver is recurrent in nature. The most common strategy adopted for training recurrent layers or networks, is during the forward pass to unroll the respective recurrent layers and use a fixed number of iterations. Then, the update of the network parameters during the backward pass is accomplished either by means of back-propagation through time (BPTT) or by its truncated version (TBPTT)~\cite{Robinson1987, Kokkinos2019}. 

Unfortunately, especially in the context of iterative solvers such an approach faces several important limitations. Among the most profound ones, is the sub-optimality of the obtained solution when the number of iterations is not large enough to ensure the convergence of the sequence of iterates. In fact, in many cases this problem cannot be circumvented easily. The reason is that if a relatively large number of unrolled iterations is utilized, then the memory requirements for storing the intermediate results of each iteration during training, can become prohibitively large. Another important challenge is the problem of vanishing/exploding gradients that frequently appear in recurrent architectures~\cite{Pascanu2013} due to the limited numerical precision of modern CPUs/GPUs, which can compromise the overall stability of the training process. In our case the problem of numerical stability is even more pronounced given that we need to repeatedly back-propagate through the eigen-decomposition in Eq.~\eqref{eq:forward_iterations}. Indeed, when the eigenvalues of the involved matrix have multiplicity greater than one, then the gradients are undefined. Therefore, severe numerical issues can appear even in the case when two of the eigenvalues are very close to each other~\cite{Wang2021}. It is also worth noting that during training we are not in position to control the behavior of the eigenvalues for each sample in the batch. Therefore, in order not to jeopardize the entire network training process, it is crucial to adopt a robust back-propagation strategy that will not be affected by this type of errors. 


%learning of geometry parameters requires backpropagation from $\bm x^\star$ into the matrix $\m A$ predicted by the preceding features extraction and matching module. We note, that $\bm x^\star$ is attained through the iterative procedure described by~\cref{eq:forward_iterations}, which has to be executed upon convergence to the minimizer of~\cref{eq:argmin_x}, and we pursue the idea of implementing this procedure as an Iterative Homogeneous Least Squares (IHLS) trainable layer. The na\"ive approach would be to represent~\cref{eq:forward_iterations} as a recurrent computational graph and then to unroll it using a pre-defined threshold on its total number of iterations. Backpropagation through time (BPTT) or its truncated version (TBPTT)~\cite{Robinson1987,Kokkinos2019} could then be employed to perform the training. We challenge such an approach, as the maximum amount of iterations for unrolling is limited by the two irremovable reasons. First of all, the prohibitively large amount of memory might be required to store the intermediate results of unrolled iterations. The second reason is related to the instabilities arising from the limited precision of numerical calculations. It results in the vanishing/exploding gradients during training of recurrent architectures ~\cite{Pascanu2013}, and unstable backpropagation through eigendecomposition $\bm u_{\text{min}}$, which in our case has to be performed for every unrolled iteration of~\cref{eq:forward_iterations}.

To overcome all the above difficulties, we exploit the fact that any limit point of the sequence of solutions $\cbr{\bm f^k}$ produced by our proposed IHLS algorithm is a stationary point. This result stems from Proposition 2.7.1 in~\cite{Bertsekas1996} and the fact that IHLS is a 
block coordinate descent minimization method and a unique solution exists for both sub-problems in Eq.~\eqref{eq:cyclic_min}. Next, we utilize the Karush-Kuhn-Tucker (KKT) optimality conditions~\cite{Boyd2004} associated with the original problem in Eq.~\eqref{eq:argmin_f}:
\bal\label{eq:stationarity_kkt}
% \nabla \br{\mc L \pr{\bm x^\star, \lambda} \equiv \rho\pr{\m A\bm x^\star;\epsilon,p} + \lambda\pr{\norm{\bm x^\star}{2}^2-1}} = ,
\nonumber \nabla_{\bm f^\star} &\br{\mc L \pr{\bm f^\star, \lambda^\star} \equiv \rho\pr{\m A\bm f^\star;\epsilon,p} + \lambda^\star\pr{\norm{\bm f^\star}{}^2-1}}\\
& = p \bm\Gamma\pr{\bm \beta^\star} \bm f^\star + 2 \lambda^\star \bm f^\star = \bm 0,
\eal
where $\mc L$ is the Lagrangian, $\lambda^*$ denotes the Lagrange multiplier and $\bm f^\star$ represents the stationary point produced by IHLS.
By multiplying both sides by ${\bm f^\star}^\transp$ and using that ${\bm f^\star}^\transp \bm f^\star = \norm{\bm f^\star}{}^2 = 1$, we can compute the corresponding Lagrange multiplier $\lambda^\star$ as:
\bal
\lambda^\star = -\frac{p}{2} {\bm f^\star}^\transp \bm\Gamma\pr{\bm \beta^\star} \bm f^\star. 
\label{eq:lagrange_multiplier}
\eal
Combining Eqs.~\eqref{eq:stationarity_kkt} and \eqref{eq:lagrange_multiplier} we end up with the following necessary condition that needs to be satisfied by the output of the IHLS layer upon convergence:
\bal\label{eq:backprop_conditions}
\bm g\pr{\bm f^\star, \bm \theta} \equiv \pr{\bm I-{\bm f^\star}{\bm f^\star}^\transp}\bm\Gamma\pr{\bm \beta^\star} \bm f^\star = \bm 0,
\eal
where the dependence on $\bm \theta$ is hidden in both $\bm f^\star$ and $\bm \beta^\star$. 

In order to be able to back-propagate through the proposed IHLS layer, we need to compute the gradient $\nabla_{\bm \theta} L = \nabla_{\bm \theta} \bm f^\star \nabla_{\bm f^\star} L$, where $L$ is the network's loss function and  $\nabla_{\bm f^\star} L$ is computed according to the chain rule and the operations involved in the  succeeding layers of IHLS in the overall network. Now, if we differentiate both sides of Eq.~\eqref{eq:backprop_conditions} w.r.t $\bm\theta$, we obtain:
\bal\label{eq:implicit_function_theorem}
&\nabla_{\bm \theta} \bm g\pr{\bm f^\star, \bm \theta} + \nabla_{\bm \theta} \bm f^\star \nabla_{\bm f^\star} \bm g\pr{\bm f^\star, \bm \theta} = \bm 0 \nonumber\\
&\Rightarrow\nabla_{\bm \theta} \bm f^\star = - \nabla_{\bm \theta} \bm g\pr{\bm f^\star, \bm \theta} \pr{\nabla_{\bm f^\star} \bm g\pr{\bm f^\star, \bm \theta}}^{-1}.
\eal
Therefore, it is possible to compute the gradient of the loss $L$ w.r.t to the set of parameters $\bm\theta$ as:
\bal\label{eq:implicit_backprop}
\nabla_{\bm \theta} L = - \nabla_{\bm \theta} \bm g\pr{\bm f^\star, \bm \theta} \pr{\nabla_{\bm f^\star} \bm g\pr{\bm f^\star, \bm \theta}}^{-1} \nabla_{\bm f^\star} L.
\eal
As a result of Eq.~\eqref{eq:implicit_backprop}, backpropagation through our IHLS layer amounts to a single vector-jacobian product (VJP) $-\nabla_{\bm \theta} \bm g\pr{\bm f^\star, \bm \theta} \bm v$, where vector $\bm v$ is obtained as the solution of a system of linear equations $\nabla_{\bm f^\star} \bm g\pr{\bm f^\star, \bm \theta} \bm v = \nabla_{\bm f^\star} L$, and $\nabla_{\bm f^\star} L$ is the incoming gradient. When our layer is applied to the fundamental matrix estimation problem, $\nabla_{\bm f^\star} \bm g\pr{\bm f^\star, \bm \theta} \in \R^{9\times9}$, meaning that the computational burden introduced by inversion of such a low-dimensional matrix is negligible. Furthermore, our derived procedure is agnostic to the number of iterations performed during the forward pass, and requires only a single backpropagation through $\bm u_{\text{min}}$ to be performed in $-\nabla_{\bm \theta} \bm g\pr{\bm f^\star, \bm \theta} \bm v$, so it lacks all of the BPTT drawbacks we have highlighted earlier. We provide a short but detailed implementation-friendly summary of our procedure in Algorithm~\ref{alg:forward} and~\ref{alg:backward}.

We note, that in Eq.~\eqref{eq:implicit_function_theorem} of our derivations we utilize the implicit function theorem, so our backpropagation strategy belongs to the emerging class of the implicit differentiation approaches~\cite{Bai2019,Zucchet2022,Gould2022}. We find our training strategy to be similar to one proposed in~\cite{Lefkimmiatis2023}, where the implicit backpropagation rules were derived for several unconstrained minimization problems. This approach is not directly applicable to our case, since in Eq.~\eqref{eq:argmin_f} we are dealing with the constrained minimization problem. 

% \begin{algorithm}[h]
% \footnotesize
%  \SetAlgoCaptionSeparator{\unskip:}
%  \SetAlgoSkip{}
%  \SetAlgoNoEnd 
%  \SetAlgoInsideSkip{}
%  \DecMargin{1cm}
% \SetKwInput{NI}{Inputs}
% \SetKwInput{Np}{Layer parameters}
% \SetKwBlock{Fwd}{Forward Pass}{}
% \SetKwBlock{Xstep}{$\bm x$-step}{}
% \SetKwBlock{Bstep}{$\bm \beta$-step}{}
% \SetKwBlock{Bwd}{Backward Pass}{}
% \NI{$\bm x_0$: initial solution, $\m A$: weighted correspondences matrix}
% \Np{$p, \epsilon$ -- robust function parameters}
% \KwResult{$\bm x^\star = \bm x^k$}
% \Fwd{
% Initialize: $k = 0$\;
% \Do{the convergence criterion is satisfied}{
% \Bstep{
% 1. Compute the residual $\bm r^k = \m A \bm x^k$.\\
% 2. Compute the vector $\bm \beta^{k+1} = \sqrt{\pr{\bm r^k}^2 + \epsilon}$, where the square and the square root are taken point-wise.
% }
% \Xstep{
% 3. Compute the normal equations matrix:
% $$
% \bm\Gamma\pr{\bm \beta^{k+1}} = \m A^\transp \pdiag{\bm \beta^{k+1}}{p-2}\m A.
% $$
% \hspace{-0.15cm}4. Find the updated solution $\bm x^{k+1}$ by solving the homogeneous least squares problem:
% $$
% \bm x^{k+1} = \bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm \beta^{k+1}}}.
% $$
% }
% $k = k+1$.
% }
% % Return $\bm x^\star = \bm x^k$.
% }
% \Bwd{
% \begin{enumerate}
% \footnotesize
% \item Define the following auxiliary computational graph on \\variables $\bm x^\star$ and $\bm \theta=\cbr{\m A, p, \epsilon}$:
% \bal\nonumber
% \hspace{-1.5cm}\bm g\pr{\bm x^\star, \bm \theta} = \bm\Gamma\pr{\bm \beta^\star} \bm x^\star - \pr{{\bm x^\star}^\transp \bm\Gamma\pr{\bm \beta^\star} \bm x^\star} \bm x^\star,
% \eal
% where $\bm\Gamma\pr{\bm \beta^\star}$ is computed from $\bm x^\star$ and $\bm \theta$ following steps \\
% 1, 2 and 3 in the \textbf{Forward Pass}.
% \item Compute $\bm v=\pr{\grad{\bm g}{\bm x^\star}}^{-1}\bm\rho$ by solving the linear system $\grad{\bm g}{\bm x^\star}\cdot\bm v = \bm \rho$, where $\bm\rho =\grad{L}{\bm x^\star}$ is the incoming gradient \\of the training loss function $L$ wrt the layer's output $\bm x^\star$.
% \item Obtain the gradient $\grad{ L}{\bm \theta}$ by computing the vector-jacobian \\product (VJP) $\grad{\bm g}{\bm \theta}\cdot\bm v$. %using any of the existing\\ auto-grad libraries (pytorch, tensorflow, ...).
% \item Use $\grad{L}{\bm \theta}$ to update the layer's parameters $p, \epsilon$ and, if\\ necessary, backpropagate to any preceding layers.
% \vspace{-.1cm}
% \end{enumerate}
% }
%  \caption{Forward and backward passes through the proposed IHLS Layer}
%   \label{alg:forward_backward}
% \end{algorithm}

\begin{algorithm}[h]
\footnotesize
 \SetAlgoCaptionSeparator{\unskip:}
 \SetKwComment{Comment}{/* }{ */}
 \SetAlgoSkip{}
 \SetAlgoNoEnd 
 \SetAlgoInsideSkip{}
 \DecMargin{1cm}
\SetKwInput{NI}{Inputs}
\SetKwInput{Np}{Layer parameters}
\SetKwBlock{Fwd}{Forward Pass}{}
\SetKwBlock{Fstep}{$\bm f$-step}{}
\SetKwBlock{Bstep}{$\bm \beta$-step}{}
\SetKwBlock{Bwd}{Backward Pass}{}
\DontPrintSemicolon
\NI{$\bm f_0, \m A$}
\Np{$p, \epsilon$}
\KwResult{$\bm f^\star = \bm f^k$}
$k \gets 0$\;
\Do{the convergence criterion is satisfied}{
\Bstep{
$\bm r^k \gets \m A \bm f^k$\;
$\bm \beta^{k+1} \gets \sqrt{\pr{\bm r^k}^2 + \epsilon}$ \Comment*[r]{square and square root are applied element-wise}
}
\Fstep{
$\bm\Gamma\pr{\bm \beta^{k+1}} \gets \m A^\transp \pdiag{\bm \beta^{k+1}}{p-2}\m A$\;
$\m U, \bm \lambda \gets \textrm{eigh}\pr{\bm\Gamma\pr{\bm \beta^{k+1}}}$\Comment*[r]{real symmetric matrix eigen-decomposition}
$\bm f^{k+1} \gets \m u_{\text{min}}$ \Comment*[r]{eigenvector of the smallest eigenvalue $\lambda_\text{min}$}
}
$k \gets k+1$.
}
 \caption{Forward pass through the proposed IHLS Layer}
  \label{alg:forward}
\end{algorithm}


\begin{algorithm}[h]
\footnotesize
 \SetAlgoCaptionSeparator{\unskip:}
 \SetKwComment{Comment}{/* }{ */}
 \SetAlgoSkip{}
 \SetAlgoNoEnd 
 \SetAlgoInsideSkip{}
 \DecMargin{1cm}
\SetKwInput{NI}{Inputs}
\SetKwInput{Np}{Buffer from Forward pass}
\SetKwBlock{Fwd}{Forward Pass}{}
\SetKwBlock{WGrad}{Record computational graph with autograd}{}
\SetKwBlock{Bstep}{$\bm \beta$-step}{}
\SetKwBlock{Bwd}{Backward Pass}{}
\DontPrintSemicolon
\NI{\grad{L}{\bm f^\star} \Comment*[r]{the incoming gradient}}
\Np{$\bm f^\star$, $\bm \theta = \cbr{\m A, p, \epsilon}$}
\KwResult{$\grad{L}{\bm \theta}$}
\WGrad{
$\bm r^\star \gets \m A \bm f^\star$\;
$\bm \beta^\star \gets \sqrt{\pr{\bm r^\star}^2 + \epsilon}$ \Comment*[r]{square and square root are applied element-wise}
$\bm\Gamma\pr{\bm \beta^\star} \gets \m A^\transp \pdiag{\bm \beta^\star}{p-2}\m A$\;
$\bm g\pr{\bm f^\star, \bm \theta} \gets \bm\Gamma\pr{\bm \beta^\star} \bm f^\star - \pr{{\bm f^\star}^\transp \bm\Gamma\pr{\bm \beta^\star} \bm f^\star} \bm f^\star$
}
$\m B \gets \frac{\partial \bm g}{\partial \bm f^\star}$ \Comment*[r]{Jacobian computed by autograd}
% $\m B \gets \m B^\transp$
$\bm v \gets {\m B}^{-\transp} \grad{L}{\bm f^\star}$\\
 $\grad{L}{\bm \theta} \gets \bm v^\transp \frac{\partial \bm g}{\partial \bm \theta}$ \Comment*[r]{VJP computed by autograd}
 \caption{Backward pass through the proposed IHLS Layer}\;
 
  \label{alg:backward}
  \vspace{-0.3cm}
\end{algorithm}

==> sections/old_algorithm.tex <==
\subsection{Iterative Homogeneous Least Squares}
\label{sec:IHLS}

In this section we describe in detail our approach for solving the optimization problem of interest. To proceed, we first rely on 
the following inequality~\cite{Sun2016}:
\bal
\abs{x}^p \le \frac{p}{2}\frac{x^2}{\beta^{2-p}} + \frac{2-p}{2}\beta^p,
\label{eq:lp_ineq}
\eal
which holds true $\forall x\in \R$, $\beta > 0$ and $0<p\le 2$.

Let us now consider the positive scalar $\sqrt{x_n^2+
\epsilon}$ with $\epsilon > 0$ being a small positive constant and plug it in \cref{eq:lp_ineq}. Then, we obtain
\bal
\pr{x_n^2+\epsilon}^{\frac{p}{2}} \le \frac{p}{2}\frac{x_n^2}{\beta_n^{2-p}}+\frac{p\epsilon}{2}\beta_n^{p-2}+ \frac{2-p}{2}\beta_n^p.
\label{eq:lp_gamma_ineq}
\eal
The above inequality is closed under summation and, thus, it further holds that:
\bal
\phi\pr{\bm x;\epsilon, p}=&\suml_{n=1}^N \pr{x_n^2+\epsilon}^{\frac{p}{2}}
\le \frac{p}{2}\bm x^\transp\pdiag{\bm\beta}{p-2}\bm x\nonumber\\
&+\suml_{n=1}^N\pr{\frac{p\epsilon}{2}\beta_n^{p-2}+\frac{2-p}{2}\beta_n^p}=\psi\pr{\bm\beta}
\eal
The image of $\psi\pr{\bm\beta}$ is strictly positive which means that:
\bal
\phi\pr{\bm x;\epsilon, p} =\min_{\bm\beta\in\R^N_+} \psi\pr{\bm\beta}.
\label{eq:var_beta}
\eal
We have thus managed to obtain a variational formulation of our robust function $\phi\pr{\bm x;\epsilon, p}$ as the minimum of a quadratic function in $\bm x$ over the auxiliary variable $\bm \beta$.

We can now switch our focus to the optimization problem of interest:
\bal
\bm x^\star = \argmin_{\norm{\bm x}{}=1}\phi\pr{\m A\bm x;\epsilon,p},
\label{eq:argmin_x}
\eal
where $\m A\in \R^{N\times 9}$ represents the matrix that holds the coordinates of the feature correspondences between a pair of images of the same scene, seen from two different views, and $\bm x=\vc{\bm F}$ is the vectorized version of the fundamental matrix $\bm F$.

Combining \cref{eq:var_beta} and \cref{eq:argmin_x} we have :
\bal
\min_{\norm{\bm x}{}=1}&\phi\pr{\m A\bm x;\epsilon,p}=\min_{\norm{\bm x}{}=1,\,\bm\beta\in\R^N_+} \psi\pr{\bm\beta} \equiv\nonumber\\&\frac{p}{2}\bm x^\transp\bm \Gamma\pr{\bm\beta}\bm x+\suml_{n=1}^N\pr{\frac{p\epsilon}{2}\beta_k^{p-2}+\frac{2-p}{2}\beta_k^p},
\label{eq:min_min}
\eal
where $\bm\Gamma\pr{\bm\beta}=\m A^\transp\pdiag{\bm\beta}{p-2}\m A$. By utilizing the variational formulation from \cref{eq:var_beta} we have achieved to end up with a joint minimization problem in the variables $\pr{\bm x, \bm \beta}$, for which it is possible to consider an alternating minimization strategy. According to this, it is straightforward to show that the optimum w.r.t $\bm x$ is obtained as the solution of a unit-norm constrained homogeneous least-squares problem:
\bal
\bm x^\star = \bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta^\star}},
\label{eq:x_argmin_beta}
\eal
where $\bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta^\star}}$ denotes the eigenvector corresponding to the smallest eigenvalue, $\lambda_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta^*}}$, of the symmetric and positive definite matrix $\bm\Gamma\pr{\bm\beta^\ast}$. Next, to obtain $\bm\beta^\star$ we need to solve the following optimization problem:
\bal
\bm\beta^\star=\argmin_{\bm\beta\in\R^N_+}\overbrace{\lambda_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta}}+\suml_{n=1}^N\pr{\frac{p\epsilon}{2}\beta_n^{p-2}+\frac{2-p}{2}\beta_n^p}}^{\mc J\pr{\bm\beta}}.
\eal
To do so, we note that for the first term of $\mc J\pr{\bm\beta}$ it holds
\bal
\lambda_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta}} =& \min_{\norm{\bm x}{}=1}\bm x^\transp \bm\Gamma\pr{\bm\beta}\bm x\nonumber\\ &\le \bm x^\transp \bm\Gamma\pr{\bm\beta}\bm x\quad\forall \bm x \mbox{ with } \norm{\bm x}{} = 1.
\eal
This upper-bound allows us to devise a majorization-minimization (MM) strategy in order to find a stationary point of the objective $\mc J\pr{\bm\beta}$ in an iterative way. Specifically, let us introduce the surrogate objective:
\bal
\mc Q\pr{\bm\beta;\bm \beta^k}\!=\!\frac{p}{2}\pr{\bm x^k}^\transp\bm\Gamma\pr{\bm\beta}\bm x^k\!+\!\suml_{n=1}^N\!\!\pr{\frac{p\epsilon}{2}\beta_n^{p-2}\!+\!\frac{2\!-\!p}{2}\beta_n^p}\!,
\eal
where $\bm x^k \equiv \bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta^k}}$. This objective function is a valid majorizer of $\mc J\pr{\bm\beta}$, since it satisfies all the necessary requirements~\cite{Hunter2004}, that is: 
\bal
\label{eq:MM_properties}
\mc Q\pr{\bm\beta;\bm \beta^k} \ge \mc J\pr{\bm \beta}, \forall \bm \beta, \bm\beta^k\,\, \mbox{and}\,\, 
\mc Q\pr{\bm \beta^k;\bm\beta^k} = \mc J\pr{\bm\beta^k}.
\eal

Based on the above, we can now find a minimizer of $\mc J\pr{\bm \beta}$ in an iterative way, as follows:
\bal
\bm\beta^{k+1} = \argmin_{\bm\beta\in\R^N_+}\mc Q\pr{\bm\beta;\bm\beta^k},
\eal
which amounts to solving the system of equations $\grad{\mc Q\pr{\bm\beta;\bm\beta^k}}{\bm\beta}=\bm 0$. It is straightforward to show that for the case of interest $0 < p \le 1$ and after simple manipulations, we finally have:
\bal
\pr{\pdiag{\m A\bm x^k}{2}+\epsilon\bm I - \pdiag{\bm\beta}{2}}\bm\beta^{p-3} = \bm 0,
\label{eq:beta_n}
\eal
where $\pr{\cdot}^{p-3}$ is applied element-wise. Given the constraint that $\beta_n > 0$, the only admissible solution of \cref{eq:beta_n} is 
\bal
\beta_n^{k+1}=\sqrt{\pr{\bm e_n^\transp\m A\bm x^k}^2+\epsilon},\,\,\forall n=1,\ldots, N
\label{eq:beta_k}
\eal
where $\bm e_n$ denotes the unit vector of the standard $\R^N$ basis, \ie all its elements are zero except to the $n$-th one which is equal to one.

Finally, by combining \cref{eq:x_argmin_beta} and \cref{eq:beta_k}, we end up with the final iterative scheme:
\bal\label{eq:forward_iterations}
\bm x^{k+1}&=\bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta^{k+1}}}\nonumber\\
&=\bm u_{\text{min}}\pr{\m A^\transp \pdiag{\pr{\m A\bm x^k}^2 + \epsilon\bm I}{\frac{p-2}{2}}\m A}.
\eal

\subsection{Network Training} %with Implicit Backpropagation}
\label{sec:backward_pass}
% Being our final goal, supervised end-to-end learning of geometry parameters requires backpropagation through the iterative procedure described by~\cref{eq:forward_iterations}. Its recurrent nature suggests us to represent it as a recurrent layer, whose parameters $\m A$ are predicted by the preceding features extraction and matching module. The resulting layer consists of three sequential operations, namely:
% \begin{itemize}
%     \item \textbf{Residual computation}, that gets as input the current estimate $\bm x^k$ and computes the residual vector $\bm r^k = \m A \bm x^k$.
%     \item \textbf{Normal equations matrix computation}, which constructs the matrix $\m A^k = \m A^\transp \pdiag{\pr{\bm r^k}^2 + \epsilon\bm I}{\frac{p-2}{2}}\m A$.
%     \item \textbf{Constrained least squares solution}, which computes the updated estimate $\bm x^{k+1} = \bm u_{\text{min}}\pr{\m A^k}$ by solving the constrained least squares with normal equations matrix $\m A^k$ by finding the eigenvector corresponding to the smallest eigenvalue of $\m A^k$.
% \end{itemize}
% We present the overall architecture of the 
Our final goal is to incorporate the IHLS solver as a layer in a wider network, which will be trained end-to-end in a supervised way. To do so, we need to be able to back-propagate efficiently through the IHLS layer. The main challenge here is that the proposed IHLS solver is recurrent in nature. The most common strategy adopted for training recurrent layers or entire networks, is during the forward pass to unroll the respective recurrent layers and use a fixed number of iterations. Then, the update of the network parameters during the backward pass is accomplished either by means of back-propagation through time (BPTT) or by its truncated version (TBPTT)~\cite{Robinson1987, Kokkinos2019}. 

Unfortunately, especially in the context of iterative solvers such an approach faces several important limitations. Among the most profound ones, is the sub-optimality of the obtained solution when the number of iterations is not large enough to ensure the convergence of the sequence. In fact, in many cases this problem cannot be circumvented easily. The reason is that if a relatively large number of unrolled iterations is used, then the memory requirements for storing the intermediate results of each iteration during training can become prohibitively large. Another important challenge is the problem of vanishing/exploding gradients that frequently appear in recurrent architectures~\cite{Pascanu2013} due to the limited numerical precision of modern CPUs/GPUs, which can compromise the overall stability of the training process. In our case this problem is even more pronounced given that we need to repeatedly back-propagate through the eigen-decomposition $\bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm\beta^{k}}}$ in \cref{eq:forward_iterations}, which can be unstable when two of the eigenvalues are very close~\cite{Wang2021}.


%learning of geometry parameters requires backpropagation from $\bm x^\star$ into the matrix $\m A$ predicted by the preceding features extraction and matching module. We note, that $\bm x^\star$ is attained through the iterative procedure described by~\cref{eq:forward_iterations}, which has to be executed upon convergence to the minimizer of~\cref{eq:argmin_x}, and we pursue the idea of implementing this procedure as an Iterative Homogeneous Least Squares (IHLS) trainable layer. The na\"ive approach would be to represent~\cref{eq:forward_iterations} as a recurrent computational graph and then to unroll it using a pre-defined threshold on its total number of iterations. Backpropagation through time (BPTT) or its truncated version (TBPTT)~\cite{Robinson1987,Kokkinos2019} could then be employed to perform the training. We challenge such an approach, as the maximum amount of iterations for unrolling is limited by the two irremovable reasons. First of all, the prohibitively large amount of memory might be required to store the intermediate results of unrolled iterations. The second reason is related to the instabilities arising from the limited precision of numerical calculations. It results in the vanishing/exploding gradients during training of recurrent architectures ~\cite{Pascanu2013}, and unstable backpropagation through eigendecomposition $\bm u_{\text{min}}$, which in our case has to be performed for every unrolled iteration of~\cref{eq:forward_iterations}.

To overcome all the above difficulties, we rely on the fact that our proposed IHLS algorithm is derived following a MM strategy and, thus, if the sequence of IHLS iterates $\bm x^k$ converges, then the limit point $\bm x^\ast$ is guaranteed to be a stationary point of the original objective function~\cite{razaviyayn2013}. 



%Instead of unrolling, we propose to perform the backpropagation based on connections between~\cref{eq:forward_iterations} and~\cref{eq:argmin_x} using other principles. We first note, that the condition $\norm{\bm x}{} = 1$ in~\cref{eq:argmin_x} could be replaced with $\norm{\bm x}{}^2 = \bm x^\transp \bm x = 1$ without affecting the minimizer. 
Next, we write the Karush-Kuhn-Tucker (KKT) optimality conditions~\cite{Boyd2004} 
that involve the Lagrangian function associated with the original problem in~\cref{eq:argmin_x}, and evaluated at the stationary point $\bm x^\star$:
\bal\label{eq:stationarity_kkt}
% \nabla \br{\mc L \pr{\bm x^\star, \lambda} \equiv \phi\pr{\m A\bm x^\star;\epsilon,p} + \lambda\pr{\norm{\bm x^\star}{2}^2-1}} = ,
\nonumber \nabla_{\bm x^\star} &\br{\mc L \pr{\bm x^\star, \lambda^\star} \equiv \phi\pr{\m A\bm x^\star;\epsilon,p} + \lambda^\star\pr{\norm{\bm x^\star}{}^2-1}}\\
& = p \bm\Gamma\pr{\bm \beta^\star} \bm x^\star + 2 \lambda^\star \bm x^\star = \bm 0.
\eal
Multiplying both sides by ${\bm x^\star}^\transp$ and exploiting that ${\bm x^\star}^\transp \bm x^\star = \norm{\bm x^\star}{}^2 = 1$, we compute the corresponding Lagrange multiplier $\lambda^\star$ as:
\bal
\lambda^\star = -\frac{p}{2} {\bm x^\star}^\transp \bm\Gamma\pr{\bm \beta^\star} \bm x^\star. 
\label{eq:lagrange_multiplier}
\eal
Combining Eqs.~\eqref{eq:stationarity_kkt} and \eqref{eq:lagrange_multiplier} we end up with a necessary condition that needs to be satisfied by the output of the IHLS layer upon convergence, that is:
\bal\label{eq:backprop_conditions}
\bm g\pr{\bm x^\star, \bm \theta} \equiv \pr{\bm I-{\bm x^\star}{\bm x^\star}^\transp}\bm\Gamma\pr{\bm \beta^\star} \bm x^\star = \bm 0,
\eal
where the dependence on $\bm \theta$ is hidden in both $\bm x^\star$ and $\bm \beta^\star$. In order to back-propagate through our IHLS solver during the network training, the gradient $\nabla_{\bm \theta} L = \nabla_{\bm \theta} \bm x^\star \nabla_{\bm x^\star} L$, where L is the network's loss function and  $\nabla_{\bm x^\star} L$ is computed according to the chain rule. 
The missing component $\nabla_{\bm \theta} \bm x^\star$ could be obtained by taking the gradient of both sides of~\cref{eq:backprop_conditions} as we show below:
\bal\label{eq:implicit_function_theorem}
&\nonumber \nabla_{\bm \theta} \bm g\pr{\bm x^\star, \bm \theta} + \nabla_{\bm \theta} \bm x^\star \nabla_{\bm x^\star} \bm g\pr{\bm x^\star, \bm \theta} = \bm 0 \Rightarrow \\
& \Rightarrow \nabla_{\bm \theta} \bm x^\star = - \nabla_{\bm \theta} \bm g\pr{\bm x^\star, \bm \theta} \pr{\nabla_{\bm x^\star} \bm g\pr{\bm x^\star, \bm \theta}}^{-1}.
\eal
As a result of our derivations, the backpropagation through our IHLS layer amounts to a single vector-jacobian product $-\nabla_{\bm \theta} \bm g\pr{\bm x^\star, \bm \theta} \bm v$, where vector $\bm v$ is obtained as the solution of a system of linear equations $\nabla_{\bm x^\star} \bm g\pr{\bm x^\star, \bm \theta} \bm v = \nabla_{\bm x^\star} L\pr{\bm x^\star}$. For the fundamental matrix estimation problem $\nabla_{\bm x^\star} \bm g\pr{\bm x^\star, \bm \theta} \in \R^{9\times9}$, meaning that the inversion of such low-dimensional matrix does not introduce any computational complexity at all. Moreover, our derived backward procedure is agnostic to the number of iterations performed during the forward pass, and requires only a single backpropagation through $\bm u_{\text{min}}$ to be performed in $-\nabla_{\bm \theta} \bm g\pr{\bm x^\star, \bm \theta} \bm v$, so it lacks all of the drawbacks we have highlighted at the beginning of~\cref{sec:backward_pass}. We provide the short but detailed implementation-friendly summary of our procedure in~\cref{alg:forward_backward}.

We note, that in~\cref{eq:implicit_function_theorem} of our derivations we utilize the implicit function theorem, so our backpropagation strategy belongs to the emerging class of the implicit differentiation approaches~\cite{Bai2019,Zucchet2022,Gould2022}. We find our training strategy to be similar to one proposed in~\cite{Lefkimmiatis2023}, where the implicit backpropagation rules were derived for several unconstrained minimization problems. This approach is not directly applicable to our case, since in~\cref{eq:argmin_x} we are dealing with the constrained minimization problem. 

\begin{algorithm}[h]
\footnotesize
 \SetAlgoCaptionSeparator{\unskip:}
 \SetAlgoSkip{}
 \SetAlgoNoEnd 
 \SetAlgoInsideSkip{}
 \DecMargin{1cm}
\SetKwInput{NI}{Inputs}
\SetKwInput{Np}{Layer parameters}
\SetKwBlock{Fwd}{Forward Pass}{}
\SetKwBlock{Bwd}{Backward Pass}{}
\NI{$\bm x_0, \m A$: weighted correspondences matrix}
\Np{$p, \epsilon$ -- robust function parameters}
\Fwd{
Initialize: $k = 0$\;
\Do{the convergence criterion is satisfied}{
1. Compute the residual $\bm r^k = \m A \bm x^k$.\\
2. Compute the vector $\bm \beta_k = \sqrt{\pr{\bm r^k}^2 + \epsilon}$, where the square and the square root are taken point-wise.\\
3. Compute the normal equations matrix:
$$
\bm\Gamma\pr{\bm \beta^k} = \m A^\transp \pdiag{\bm \beta^k}{p-2}\m A.
$$
\hspace{-0.15cm}4. Find the updated solution $\bm x^{k+1}$ by solving the homogeneous least squares problem:
$$
\bm x^{k+1} = \bm u_{\text{min}}\pr{\bm\Gamma\pr{\bm \beta^k}}.
$$
\hspace{-0.15cm}5. $k = k+1$.
}
Return $\bm x^\star = \bm x^k$.
}
\Bwd{
\begin{enumerate}
\footnotesize
\item Define the following auxiliary computational graph on \\variables $\bm x^\star$ and $\bm \theta=\cbr{\m A, p, \epsilon}$:
\bal\nonumber
\hspace{-1.5cm}\bm g\pr{\bm x^\star, \bm \theta} = \bm\Gamma\pr{\bm \beta^\star} \bm x^\star - \pr{{\bm x^\star}^\transp \bm\Gamma\pr{\bm \beta^\star} \bm x^\star} \bm x^\star,
\eal
where $\bm\Gamma\pr{\bm \beta^\star}$ is computed from $\bm x^\star$ and $\bm \theta$ following steps \\
1, 2 and 3 in the \textbf{Forward Pass}.
\item Compute $\bm v=\pr{\grad{\bm g}{\bm x^\star}}^{-1}\bm\rho$ by solving the linear system $\grad{\bm g}{\bm x^\star}\cdot\bm v = \bm \rho$, where $\bm\rho =\grad{L}{\bm x^\star}$ is the incoming gradient \\of the training loss function $L$ wrt the layer's output $\bm x^\star$.
\item Obtain the gradient $\grad{ L}{\bm \theta}$ by computing the vector-jacobian \\product (VJP) $\grad{\bm g}{\bm \theta}\cdot\bm v$. %using any of the existing\\ auto-grad libraries (pytorch, tensorflow, ...).
\item Use $\grad{L}{\bm \theta}$ to update the layer's parameters $p, \epsilon$ and \\backpropagate further into the parents of $\m A$.
\vspace{-.1cm}
\end{enumerate}
}
 \caption{Forward and backward passes through the proposed IHLS Layer}
  \label{alg:forward_backward}
\end{algorithm}
